DeltaLCA: Comparative Life-Cycle Assessment for Electronics Design

Reducing the environmental footprint of electronics and computing devices requires new tools that empower designers to make informed decisions about sustainability during the design process itself. This is not possible with current tools for life cycle assessment (LCA) which require substantial domain expertise and time to evaluate the numerous chips and other components that make up a device. We observe first that informed decision-making does not require absolute metrics and can instead be done by comparing designs. Second, we can use domain-specific heuristics to perform these comparisons. We combine these insights to develop DeltaLCA, an open-source interactive design tool that addresses the dual challenges of automating life cycle inventory generation and data availability by performing comparative analyses of electronics designs. Users can upload standard design files from Electronic Design Automation (EDA) software and the tool will guide them through determining which one has greater carbon footprint. DeltaLCA leverages electronics-specific LCA datasets and heuristics and tries to automatically rank the two designs, prompting users to provide additional information only when necessary. We show through case studies DeltaLCA achieves the same result as evaluating full LCAs, and that it accelerates LCA comparisons from eight expert-hours to a single click for devices with ~30 components, and 15 minutes for more complex devices with ~100 components.

==> description.tex <==
Figure 1: An overview diagram of the LabelAId system, which contains one, a novel ML-based pipeline for detecting labeling mistakes, which is efficiently trained to infer label correctness based on user behavior and domain knowledge; and two, a real-time ML model and UI that tracks worker behavior and intervenes when an inferred mistake is occurring. LabelAId improves data quality and worker expertise by providing just-in-time feedback during crowdsource labeling.

Figure 2: Conceptual diagram of our LabelAId pipeline. Programmatic weak supervision, utilizing domain-specific knowledge and heuristics, is employed to annotate the raw data. Subsequently, the noisy labels generated from PWS are used to pre-train the inference model. Lastly, the inference model is fine-tuned using clean labels for the target downstream task.

Figure 3: This figure showcases the Project Sidewalk Labeling Interface. Part A displays the interface used for labeling. Part B lists the different types of labels that can be applied, such as "obstacle" or "clear path." Part C provides examples of severity ratings for surface problems, ranging from 1 to 5, with 5 being the most severe and indicating a surface impassable for wheelchair users.

Figure 4: Conceptual diagram of our FT-Transformer-based model architecture. First, the model transforms the hybrid features (e.g., two numerical and two categorical features) into unified embeddings. Subsequently, these embeddings are processed iteratively by the Transformer layer. The final output is based on the [CLS] token.

Figure 5: Overall performance of our LabelAId pipeline compared to the traditional ML methods as the number of clean downstream labels increases. Note that the x-axis is on a log scale (N = 3, error bar = $\pm\sigma$). Each baseline model is trained on 50, 100, 200, 500, and 1000 clean labels from Seattle $\mathcal{D}_c$. The pre-trained FT-Transformer is fine-tuned on the equivalent number of clean downstream samples.

Figure 6: Selected typical inference false positives per label type, where the model incorrectly infers the label as correct when, in fact, the label is wrong. a, c, failed to differentiate between a curb ramp and a missing curb ramp. b, d, labeled a drainage swale near an intersection with no sidewalk. d-j, label has attributes for a correct label but there is ample space for a wheelchair user to pass. 

Figure 7: Selected typical inference false negatives per label type, where the model incorrectly infers the label as wrong when, in fact, the label is correct. a, absent geospatial information for certain roads. b-d, labeled mid-block crossings. e-h, missed optional input or change of GSV. i, j, rated Missing Sidewalk as passable.

Figure 8: This Figure illustrates the user flow diagram of LabelAId when implemented in Project Sidewalk. The process starts with a user placing a label using the Project Sidewalk interface. If LabelAId detects an error, a just-in-time intervention dialog appears. The user then has three options: keep the label, delete the label, or view common mistakes related to that label type. If the user chooses to view common mistakes, they can also navigate to a page showing correct examples.

Figure 9: This figure contains system screenshots of LabelAId as implemented in Project Sidewalk. Part A shows a pop-up dialog that appears when a user label error is detected, featuring a mistake title, rotating labeling tips, and three action buttons: "Yes, I am sure," "No, remove the label," and "View Common Mistakes." Parts B and C are screenshots of the Common Mistakes Page and Correct Examples Page, respectively. Both pages display the user's current label alongside 3-4 example labels for easy comparison.

Figure 10: This description presents data on user labeling precision. Part A features a raincloud plot, which combines a half violin plot and a box plot, to illustrate the difference in label precision between a control group and an intervention group. This is shown for overall precision and for five specific label types. Part B is a table that lists the mean, standard deviation, Mann-Whitney U value, and p-value for both groups. The table indicates that the intervention group had statistically significantly higher precision in the overall category, as well as for the "curb ramp" and "no curb ramp" label types.

==> supplementart-materials.tex <==
There are three supplementary materials:

1- "orientation-slides.pdf" is a PDF containing the orientation presentation during user studies. 

2- "post-study-questionnaire.pdf" is a PDF that contains the pre-study questionnaire questions.

3- "post-study-questionnaire.pdf" is a PDF that contains the post-study questionnaire questions.
